Exploiting Boosting in Hyperdimensional Computing for Enhanced Reliability in Healthcare

Hyperdimensional computing (HDC) enables efficient data encoding and processing in high-dimensional space, benefiting machine learning and data analysis. However, underutilization of these spaces can lead to overfitting and reduced model reliability, especially in data-limited systems a critical issue in sectors like healthcare that demand robustness and consistent performance. We introduce BoostHD, an approach that applies boosting algorithms to partition the hyperdimensional space into subspaces, creating an ensemble of weak learners. By integrating boosting with HDC, BoostHD enhances performance and reliability beyond existing HDC methods. Our analysis highlights the importance of efficient utilization of hyperdimensional spaces for improved model performance. Experiments on healthcare datasets show that BoostHD outperforms state-of-the-art methods. On the WESAD dataset, it achieved an accuracy of 98.37%, surpassing Random Forest, XGBoost, and OnlineHD. BoostHD also demonstrated superior inference efficiency and stability, maintaining high accuracy under data imbalance and noise. In person-specific evaluations, it achieved an average accuracy of 96.19%, outperforming other models. By addressing the limitations of both boosting and HDC, BoostHD expands the applicability of HDC in critical domains where reliability and precision are paramount.

==> Chapters/0_abstract.tex <==
\begin{abstract}
    Hyperdimensional Computing (HDC) represents a promising field in artificial intelligence, optimized for hardware friendly design. However, the exploration of its theoretical foundations and practical applications remains somewhat limited. A particular area of concern is the underutilization of the high-dimensional spaces in which vectors are represented. This oversight can lead to overfitting, potentially reducing the reliability of models in data-constrained systems and capping their performance. This issue becomes critically limiting in sectors where safety is paramount, such as in healthcare, where the demands for noise robustness, stability, and consistent performance are non-negotiable. In response to these challenges, we propose BoostHD, a novel strategy aimed at optimizing the use of high-dimensional spaces by integrating the concepts of boosting and HDC. BoostHD applies a boosting algorithm to partition the traditional high-dimensional space into subspaces, thereby assembling an ensemble model composed of multiple weak learners. Our research shows that by harnessing the synergistic potential between boosting techniques and HDC, BoostHD elevates performance limits and achieves reliability compared to existing HDC methodologies, expanding the domain of the HDC.
\end{abstract}
